Extreme value methods for estimating rare events in Utopia

To capture the extremal behaviour of complex environmental phenomena in practice, flexi\-ble techniques for modelling tail behaviour are required. In this paper, we introduce a variety of such methods, which were used by the Lancopula Utopiversity team to tackle the EVA (2023) Conference Data Challenge. This data challenge was split into four challenges, labelled C1-C4. Challenges C1 and C2 comprise univariate problems, where the goal is to estimate extreme quantiles for a non-stationary time series exhibiting several complex features. For these, we propose a flexible modelling technique, based on generalised additive models, with diagnostics indicating generally good performance for the observed data. Challenges C3 and C4 concern multivariate problems where the focus is on estimating joint extremal probabilities. For challenge C3, we propose an extension of available models in the multivariate literature and use this framework to estimate extreme probabilities in the presence of non-stationary dependence. Finally, for challenge C4, which concerns a 50 dimensional random vector, we employ a clustering technique to achieve dimension reduction and use a conditional modelling approach to estimate extremal probabilities across independent groups of variables.

==> LaTeXFiles/preamble.tex <==
%Packages
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{natbib} 
\usepackage{url} 
\usepackage{pdflscape}
\usepackage{setspace}
\usepackage{multirow}
\usepackage{hyperref}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{bbm} 
\RequirePackage[dvipsnames]{xcolor}
% \usepackage{breqn}
\usepackage{xcolor}
\usepackage{bm}
\usepackage{authblk}
\usepackage{mathptmx}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{nccmath}
\usepackage{mathrsfs}

% Checking something - Lídia
\usepackage{setspace}
\usepackage{etoolbox}
\usepackage{environ} 
\usepackage{soul}

% Define a new environment for equations with modified line spacing
\NewEnviron{myequation}{%
    \begin{equation}
    \setstretch{1.5}
    \BODY
    \end{equation}
}
\NewEnviron{myequation*}{%
    \begin{equation*}
    \setstretch{1.5}
    \BODY
    \end{equation*}
}

% \NewEnviron{myalign}{%
%     \vspace{-0.5cm}
%     $$\begin{array}{rcl}
%     \BODY 
%    %\setstretch{1.25}
%     \end{array}$$
% }

% \NewEnviron{myalign*}{%
%     \vspace{-0.5cm}
%     $$\begin{array}{rcl}
%     \BODY 
%    %\setstretch{1.25}
%     \end{array}$$
% }

% \NewEnviron{myalign1}{%
%     \vspace{-0.5cm}
%     \begin{align}
%     \setstretch{1.25}
%     \BODY
%     %    \vspace{-1cm}
% \end{align}
% }

% \NewEnviron{myalign1*}{%
%     \vspace{-0.5cm}
%     \begin{align*}
%     %\setstretch{1.25}
%     \BODY 
%    \setstretch{1.25}
%     \end{align*}
% }

% \newcommand{\equationlinespread}{1.25} 
% \newcommand{\alignlinespread}{1.25} 

%Setting margins
% DON'T change margins - should be 1 inch all around.
\addtolength{\oddsidemargin}{-.5in}%
\addtolength{\evensidemargin}{-1in}%
\addtolength{\textwidth}{1in}%
\addtolength{\textheight}{1.7in}%\\
\addtolength{\topmargin}{-1in}%

%Numbering for equations
\numberwithin{equation}{section}

%Defining new commands
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\Tau}{\mathrm{T}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\def\spacingset#1{\renewcommand{\baselinestretch}%
{#1}\small\normalsize} \spacingset{1}

\def\CB#1{{\textcolor{Green}{[CB: #1]}}}
\def\CBnew#1{{\textcolor{Cyan}{ #1}}}

\def\ED#1{{\textcolor{Red}{[ED: #1]}}}
\def\LA#1{{\textcolor{brown}{[LA: #1]}}}
\def\LAcorr#1{{\textcolor{orange}{#1}}}
\def\CM#1{{\textcolor{blue}{[CM: #1]}}}
\def\LK#1{{\textcolor{WildStrawberry}{[LK: #1]}}}
\def\MS#1{{\textcolor{Purple}{[MS: #1]}}}
\def\DH#1{{\textcolor{Plum}{[DH: #1]}}}
\def\RC#1{{\textcolor{magenta}{[RC: #1]}}}
\def\AF#1{{\textcolor{Mahogany}{[AF #1]}}}
\def\AFnew#1{{\textcolor{Teal}{ #1}}}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{property}{Property}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\renewcommand\Affilfont{\small\color{black}}

%Bibliography style
\bibliographystyle{LaTeXFiles/adapted_apalike.bst}

==> Sections/C1C2/bootstrapping.tex <==
For each of the 100 different covariate combinations, $\boldsymbol x_i$ for $i\in\{1,\ldots,100\}$, we need to construct central 50\% confidence intervals. We use a bootstrapping procedure to avoid making potentially inaccurate assumptions, for example assumptions such as the asymptotic normality approximation of maximum likelihood estimates. Traditional bootstrap approaches are non-parametric and randomly resample the data with replacement. However, in Section~\ref{subsec:edac1andc2} we find that the response variable is dependent on covariates, and these covariates exhibit temporal dependence. A standard bootstrap procedure would not reflect this dependence. We preserve the temporal dependence structure of covariates and their relationship with the response variable by approximating our confidence intervals using the stationary, semi-parametric bootstrapping procedure adopted by~\cite{DArcy2023}.

First, the response variable $Y_t$ is transformed to Uniform(0,1) margins; denote this sequence $U_t^Y=F_{Y_t|\tilde{\boldsymbol X}_t}(Y_t|\tilde{\boldsymbol{X}}_t=\boldsymbol \tilde x_t)$ where $F_{Y_t|\tilde{\boldsymbol X}_t}$ is the estimated model~\eqref{eq:C1_model}. We then adopt the stationary bootstrap procedure of~\cite{Politis1994} to retain the temporal dependence in the response and explanatory variables. The block length $L$ is simulated from a Geometric$(1/l)$ distribution, where the mean block length $l\in\mathbb{N}$ is carefully selected based on the autocorrelation function. This was selected at 50 days, the maximum lag for which the autocorrelation was significant across all variables; see the Supplementary Material. Denote this bootstrapped sequence on Uniform margins by $U_t^B$. We transform  $U_t^B$ back to the original scale using our fitted model, preserving the original structure of $Y_t$; we denote this series $Y_t^B$. Then we fit our model to $Y_t^B$ to re-estimate all of the parameters and thus the quantile of interest. We repeat this procedure to obtain 200 bootstrap samples. %\LA{do we need to say why we chose 200 samples?}

==> Sections/C1C2/exploratory_analysis.tex <==
%This section details our exploratory analysis for challenges C1 and C2. 
We were informed that the response variable $Y_{t},\; t \in \{1,\hdots,n\},$ is independent over time \citep{Rohrbeck2023}, but is affected by the covariate vector $\boldsymbol{X_t}=\{V_{1,t},\ldots,V_{8,t}\}$. However, it is not clear which covariates affect $Y$, and what form these covariate-response relationships take. In what follows, we aim to explore these relationships so we can account for them in our modelling framework. 

%Both challenges concern 70 years of daily data for the city of Amaurot. Note that years have 12 months of 25 days. \textcolor{red}{The environmental response variable $Y$ is denoted $Y_{1,t}$ for site 1 (Amaurot) and day $t=1,\ldots,n$; for the remainder of this section we use $Y_t$ for simplicity as we are only concerned with Amaurot.} We have eight potential explanatory variables \CM{Move to intro}$\bm X_{t}=\{V_{1,t},\ldots,V_{8,t}\}$ where $V_1,\ldots,V_4$ are unnamed covariates that are assumed to be IID, and $V_5,\ldots,V_8$ correspond to season ($S1$ for months $1,\ldots,6$ and $S2$ for months $7,\ldots,12$), wind speed, wind direction and atmosphere. In figures and expressions, we henceforth denote as $S$, $WS$, $WD$ and $A$, respectively. This notation follows from~\cite{Rohrbeck2023}.

To begin, we explore the dependence between all variables to understand the relationships between covariates, as well the relationships between individual covariates and the response variable. We investigate dependence in the main body of the data using Kendall's $\tau$ measure, while for the joint tails, we use the pairwise extremal dependence coefficients $\chi$ and $\eta$ defined in Section~\ref{subsec::background_EVA}; values for all pairs are shown in Figure~\ref{fig:dep_heat}, with the threshold $u$ set at the empirical 0.95-quantile for the extremal measures. %Recall that for $\chi\in(0,1)$, the two variables are asymptotically dependent (AD) whilst $\chi=1$ corresponds to asymptotic independence (AI). Whilst, $\overline\chi=1$ and $\overline\chi<1$ correspond to asymptotic dependence \AF{AD now we have defined} and asymptotic independence \AF{AI}, respectively. 


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/Eleanor/Heatmap_dependence_v2.pdf}
    \caption{Heat maps for dependence measures for each pair of variables: Kendall's $\tau$ (left), $\chi$ (middle) and $\eta$ (right). Note the scale in each plot varies, depending on the support of the measure, and the diagonals are left blank, where each variable is compared against itself.}
    \label{fig:dep_heat}
\end{figure}

The response variable $Y$ has the strongest dependence with $V_3$ in the body of the distribution, followed by $V_6$ (wind speed) then $V_7$ (wind direction). Similarly, $Y$ has strong dependence with $V_2$, $V_3$ and $V_6$ in the tail. We also find strong dependence between $V_6$ and $V_7$ in the body, but evidence of weak dependence in the tail (dark blue for $\hat\chi$ and $\hat\eta$). There is also strong dependence between $V_1$ and $V_2$ in both the body and tail (see dark red for $\hat\eta$). We find very similar dependence relationships when the data are split into seasons. In the Supplementary Material, we show scatter plots of each covariate against the response variable; these demonstrate a highly non-linear relationship for each explanatory variable with $Y$.

%Since $V_6$ and $V_7$ have strong relationships with the response variable $Y$, we explore these variables in more detail. The most notable feature of both variables is that they have a significant shift in distribution. We use the \verb|changepoint| package~\citep{Killick2014} in \verb|R| to estimate the difference in mean for both variables; just 5 observations separate the estimated changepoints, so we assume the changes occur simultaneously. Before the changepoint, winds typically occur in the southwest direction and are greater in magnitude, while after the changepoint, they occur mainly in the northeast direction and are lower in magnitude; see the Supplementary Material.~\citet{Rohrbeck2023} state this non-stationarity was created unintentionally when designing the data challenge.

Next, we explore temporal relationships for the response variable $Y$. We first find temporal non-stationarity in that the distribution of $Y$ varies significantly with $V_5$ (season); see the Supplementary Material for more detail. The magnitude of $Y_t$ is higher for season 1 than season 2, in both the main body and tail of the distribution. However, within each season, across months, there is little temporal variation in the distribution of $Y$. We also find that $Y$ exhibits temporal independence at all lags, with acf values close to zero (see the Supplementary Material). 

%We also explore temporal dependence in the covariates.~\cite{Rohrbeck2023} states that $V_1,\ldots,V_4$ are temporally independent. We find that for $V_6$ and $V_7$, the acf remains significantly different from zero at all time lags (see the Supplementary Material) due to the changepoint discussed earlier. Finally, $V_8$ has high acf values at the earliest lags that decrease rapidly until lag 25 (i.e., the length of a month) and then continue to decrease at a slower rate until $\sim50$ time lags. This is because atmosphere is recorded monthly.

As noted in \citet{Rohrbeck2023}, 11.7\% of the observations have at least one possible predictor variable missing completely at random (MCAR). A detailed breakdown of the pattern of missing predictor observations is provided in the Supplementary Material. Since we can assume the data are MCAR, ignoring the observations that have a missing predictor variable will not bias our inference. However, a complete case analysis is undesirable due to the amount of data loss. To mitigate against this, we attempt to impute the observations where predictors are missing but ultimately found a case analysis approach works best for our data. This results in only 4\% of observations being removed for our final model.

==> Sections/C1C2/intro.tex <==
%%%%%%%%% ------- BACKGROUND ------- %%%%%%%%%%
%This section discusses our approach for challenges C1 and C2 in the univariate setting. 
Both challenges concern 70 years of daily data for the capital city of Amaurot. Each year has 12 months of 25 days and two seasons (season 1 for months 1-6, and season 2 for months 6-12). Suppose $Y$ is an unknown response variable, and $\boldsymbol{X}=(V_{1},\ldots, V_{8})$ is a vector of covariates, $(V_1, V_2, V_3, V_4)$ denoting unknown environmental variables and $(V_5,V_6,V_7,V_8)$ denoting season, wind direction (radians), wind speed (unknown scale), and atmosphere (recorded monthly), respectively. 

For C1, we build a model for $Y \mid \boldsymbol{X}$ \RC{using an extenton to the GPD \eqref{eqn:gpd_non_stationary}} and estimate the 0.9999-quantile, with associated 50\% confidence intervals, for 100 different covariate combinations denoted $\boldsymbol x_i$ for $i \in \{1,\ldots,100\}$. Note $\boldsymbol{x}_i$ are not covariates observed within the data set, but new observations provided by the challenge organisers.

For C2, we estimate the marginal quantile $q$ such that $\Pr(Y>q)=(6\times10)^{-4}$, which corresponds to a once in 200 year event in the IID setting. Therefore, we first estimate the marginal distribution $F_{Y}(y)$ using Monte-Carlo techniques; see for instance,~\cite{Eastoe2009}. Since we have a large sample size $n=21,000$ it is reasonable to assume that the observed covariate sample is representative of $\boldsymbol{X}$. We can approximate the marginal distribution as follows,
\begin{myequation}
    \hat F_{Y}(y)=\int_{\boldsymbol{X}} F_{Y\mid{\boldsymbol{X}}}(y\mid\boldsymbol{x})f_{\boldsymbol{X}}(\boldsymbol{x})\mathrm{d}\boldsymbol{x}\approx \frac{1}{n}\sum\limits_{t=1}^{n} F_{Y_t\mid{\boldsymbol{X}_t}}(y_t\mid\boldsymbol{x}_t).\label{eq:MC_dist}
\end{myequation} To approximate $F_Y(y)$, we first re-estimate the GPD parameters, now using a penalised log-likelihood which incorporates the following loss function, provided by the challenge organisers,
\begin{myequation}
\mathcal{L}(q,\hat{q}) = 
    \begin{cases}
        0.9(0.99q - \hat{q})&\text{if }\, 0.99q>\hat{q},\\
        0 &\text{if }\, \left|q-\hat{q}\right|\leq 0.01q,\\
        0.1(\hat{q}-1.01q)&\text{if }\, 1.01q<\hat{q},
    \end{cases}
    \label{eq:loss_fn}
\end{myequation} where $q$ and $\hat{q}$ are the true and estimated marginal quantiles, respectively. This loss function penalises under-estimation more heavily than an over-estimation. 

We conduct the same EDA for both challenges given the same covariates are used; this is outlined in Section~\ref{subsec:edac1andc2}. In Section~\ref{section:model_development} we introduce our techniques for modelling $Y \mid \boldsymbol{X}$, which is then used for modelling $Y$ via~\eqref{eq:MC_dist}. Our approach for uncertainty quantification is outlined in Section~\ref{section:uncertainty}, and we give our results for both challenges in Section~\ref{section:resultsc1andc2}.

==> Sections/C1C2/missing_data.tex <==
    %\subsubsection{Missing data}

    %edit this down to only include pertinent bits
    %e.g. Missing data we could use MCAR and MAR

        % As noted in \citet{Rohrbeck2023}, 11.7\% of the observations have at least one possible predictor variable $(V_{1}, V_{2}, V_{3}, V_{4}, V_{6}, V_{7})$ missing completely at random (MCAR). Most of the predictor observations are missing on their own, for example, $V_{4}$ is missing 407 times whilst there are only 119 instances of two or more of the predictors missing simultaneously. A detailed breakdown of the pattern of missing predictor observations is provided in the Supplementary Material. 
        
        % The missing observations must be accounted for before implementing a modelling framework, as failing to do so could bias the inference. Since we can assume the data are MCAR, ignoring the observations that have a missing predictor variable will not result in bias. Note, if the data were not MCAR this would not be the case and the missing values would need greater consideration (see \citet{Little2019} for more details). However, in this scenario a complete case analysis could be used. This is undesirable though as we will lose valuable information about the extremes of the response. To try and retain the observations where predictors are missing, we investigate several methods to replace, \textquotedblleft impute\textquotedblright, the missing values.
        
        %Let $\mathbf{X}$ be an $(n \times d)$ rectangular data set, where $x_{i,j}$ is the value of the $i^{\text{th}}$ observation of the $X_{j}$ random variable, for $i = 1, \hdots, n$, and $j = 1, \hdots, d$. Let $\mathbf{M}$ also be an $(n \times d)$ matrix such that $m_{i,j} = 1$, if $x_{i,j}$ is observed and $m_{i,j} = 0$ if $x_{i,j}$ is missing. Assume that we fit a model with parameters $\boldsymbol{\theta}$, then we say that under an MCAR assumption, the missing data is independent of the observed data, i.e., $f(\mathbf{M} \mid \mathbf{X}, \boldsymbol{\theta}) =  f(\mathbf{M} \mid \boldsymbol{\theta})$, for all $\mathbf{M}$ and $\boldsymbol{\theta}$.
        %\CB{Again, we need consistency with notation. Make sure $X$ also used in the precious section}

        % If the probability of the missing data only depends on the data that we have already observed and not on the other data that is missing, then this type of missing data is termed missing at random (MAR). Define $\mathbf{X}_{\text{obs}}$ as the random variables we observe and $\mathbf{X}_{\text{miss}}$ as the random variables that have missing values, then the above can be written in terms of its density as
        % \[
        %     f(\mathbf{M} \mid \mathbf{X}, \boldsymbol{\theta}) =  f(\mathbf{M} \mid \mathbf{X}_{\text{obs}}, \boldsymbol{\theta}),
        % \]
        % for all $\mathbf{X}_{\text{miss}}$ and $\boldsymbol{\theta}$. An example of this is if a sensor is unable to record an accurate temperature because it is too hot or cold.
        
        % Finally, if data is not MCAR or MAR, then it is defined as missing not at random (MNAR). This is where the probability of data being missing depends on the missing values. This is common in longitudinal data analysis and clinical trials where patients stop coming to check-ups because they are too ill to do so.

        % Figure \ref{fig:230811_Missing_Data} shows the number of times a covariate is missing individually and simultaneously with other covariates e.g., V3 is missing on its own 357 times and is missing at the same time as Wind Speed on 12 occurrences. We assume the data are MCAR so ignoring missing values will not bias our inference. As such, a complete case analysis could be used, but this results in a loss of 11.7\% of the data. This contains valuable information about the extremes of the response so it is undesirable to discard it \ED{We don't know that missing data are extreme (?) so maybe rephrase to 'this could contain valuable..'}. To try and retain the data we investigated several methods to replace, \textquotedblleft impute\textquotedblright, the missing values. 
        
        % There are numerous methods for imputing missing data; see \citet{Little2019} for details. Since we are concerned with modelling extreme values, we want the imputation model to: 1) capture the marginal distribution of the predictors; 2) impute values in the tail of the marginal and joint distributions; and 3) retain the extremal dependence structure between the predictors and response. We attempt several methods of imputation such as a non-parametric (random forest) predictive mean matching approach using Multiple Imputation by Chained Equations \citep{vanBuuren2011}, and a copula-based approach proposed by \citet{DiLascio2015}. \CB{Do we need all of this detail given we don't use any of this stuff in our approach? Also, these references seem rather niche} \AF{We can get rid if push comes to shove, I think the detail was to say if you are going to impute data with extremes this is what you need to care about and more this is an open-research topic in the area.} Neither approach is satisfactory as the former fails to satisfy all the aims, and the latter fails to satisfy 3). Other imputation methods are available that may yield more satisfactory results. Since our aims could not be met, we elect not to impute the data. Rather than a complete case analysis, we use a case analysis approach to mitigate the loss of information, i.e., an observation will only be removed if the predictor is included in our model and is missing. This results in only 4.0\% of the data being discarded for our final model.
        
        % The big question is, why do we care about missing data? The type of missing data impacts the inference and if the underlying mechanism that is causing the missing data is ignored then this can lead to biased parameter estimates. For instance, if the missing values in the MAR example are ignored, then the probability of observing data outside the range of the observed data will be lower than it should be. The only time is acceptable to ignore missingness is when data is MCAR, as it does not depend on the data, meaning the inference will be unbiased. However, this can result in a large portion of data being removed from the analyses which could be undesirable.

        % The data provided in the data challenge is simulated and has been random perturbed so that the missing data is MCAR. The data consists of 70 years of daily observations, where a year consists of 12 months and a month consists of 25 days, resulting in a total of 21,000 observations. Figure \ref{fig:230811_Missing_Data} shows the number of times a random variable is missing individually and simultaneously with other random variables e.g., V3 is missing on its own 357 times and is missing at the same time as Wind Speed on 12 occurrences. Since the data is MCAR, we could remove all observations where a value is missing for one or more of the random variables (known as complete case analysis), however, this would result in 11.7\% of the data being discarded which could contain useful information. Therefore, we investigated several method to replace, \textquotedblleft impute\textquotedblright, the data using the other available data.

    %     \begin{figure}
    %         \centering
    %         \includegraphics[scale = 0.7]{Figures/Aiden/230811_Missing_Data.pdf}
    %         \caption{Number of times random variables are missing in the data. \ED{Move to SM since it's quite big? Summarize in text.} \CB{Agreed. Also, make sure not to have the `_NA' notation, as this is not defined in the text}}
    %         \label{fig:230811_Missing_Data}
    %     \end{figure}

    % \subsubsection{Imputation}
    %     \ED{If we are struggling for room, this section could go to supplementary since we didn't use imputation, but I'd like to leave it in if we can so let's see how we go!} \CB{Going to sound brutal here, and I can see a lot of work has gone into this... but this subsection probably isn't worth including if we didn't use imputation. Can summarise in two lines - one saying we tried imputation and it didn't work because of a, b, and c, then the other line saying we removed all rows where covariates of interest were missing. Emphasise that since only 4\% of data was discarded, this probably had very little affect on the overall fit. }
        
    %     There are numerous methods for imputing missing data \citep{Little2019, Rubin2004}. Since we are concerned with extreme value modelling, we want to impute values in the tail of the distribution, and retain the dependence structure between covariates and response. Common \textquotedblleft ad hoc\textquotedblright \; approaches will fail to do this, therefore, we attempted to a use Multiple Imputation by Chained Equations (MICE) \citep{vanBuuren2011}. 
    %     % Common \textquotedblleft ad hoc\textquotedblright \; methods include: hot deck imputation \citep{2002_Marker} where missing values are replaced with values from similar observations based on the other observed random variables, although \citet{2010_He} notes that the method tends to result in an underestimation of variances; last observation carried forward (or next observation carried back) \citep{2016_Liu} where the previous (next) observation is used to fill in a missing value, although this can result in bias, particularly if the data is missing not at random \citep{2016_Lachin}; and mean substitution \citep{2016_Liu} where missing values for a random variable are substituted with its mean. All these methods do not impute the extremes of a random variable very well, therefore, we attempt to use more explicit modelling techniques.

    %     % By explicit modelling techniques, we mean that we want to impute the missing data using a posterior predictive distribution, i.e.,
    %     % \[
    %     %     f(\mathbf{X}_{\text{miss}} \mid \mathbf{X}_{\text{obs}}) = \int f(\mathbf{X}_{\text{miss}} \mid \mathbf{X}_{\text{obs}}, \boldsymbol{\theta}) f(\boldsymbol{\theta} \mid \mathbf{X}_{\text{obs}}) d\boldsymbol{\theta}
    %     % \]
    %     % For more details on how to draw such samples please see \citet{2004_Rubin}. Imputation performed in this manner is usually undertaken using a regression or a stochastic regression model to add additional uncertainty in the predicted values.

    %     % Due to there being large levels of uncertainty in the imputed values, it is common practice now to use multiple imputation techniques which are no longer problematic due to their large computational costs. This involves creating multiple data sets, $m$, each of which is analysed and the parameters of interest is pooled from the $m$ fitted models. \citet{2004_Rubin} suggests that even moderate levels of $m$, say 10, is enough. Given the large proportion of data missing in our case, and the complex relationships in the data, we only investigated methods that utilise multiple imputation.

    %     % The most common method for imputing missing data in the multivariate setting is Multiple Imputation by Chained Equations (MICE) \citep{2011_vanBuuren}. 
    %     The default approach within MICE is the predictive mean matching (PMM) method proposed by \citet{Little1988}. There is an underlying assumption that the data follows a multivariate Gaussian distribution, however, this can be relaxed by using a non-parametric approach, specifically a random forest. Utilising MICE for our data resulted in poor marginal imputation as the extremes of the covariates \ED{Not sure on `extremes of covariates'} were not imputed well; this is a limitation of MICE as it is unable to impute outside the range of observed values and because it tries to match the mean of the predictive posterior with the mean of the observed samples \ED{Is because needed?} \DH{I wonder is there some reference that supports our finding that extremes are hard to impute in general?}. In addition, the \DH{extremal }dependence structure was not retained \DH{which is an important feature of the data to be modelled in C3-4}. Figure \ref{fig:230813_Y_V3_Joint_Density} shows this with the contour plots from joint distribution of the observed values of \emph{Y} and \emph{V3} in the top left being very different to the contours of the imputed values with the most notable difference being that simultaneously large values of \emph{Y} and \emph{V3} are practically absent in the imputed data sets. \ED{For brevity: Figure \ref{fig:230813_Y_V3_Joint_Density} shows that the joint distribution of the observed values of \emph{Y} and \emph{V3} is significantly different to the imputed values, with the most notable difference being that simultaneously large values of \emph{Y} and \emph{V3} are practically absent in the imputed data sets.}

    %     \begin{figure}
    %         \centering
    %         \includegraphics[scale = 0.65]{Figures/Aiden/230813_Y_V3_Joint_Density.pdf}
    %         \caption{Joint density contour plots of \emph{Y} and \emph{V3} of observed values in the top left and imputed data sets using the PMM method.}
    %         \label{fig:230813_Y_V3_Joint_Density}
    %     \end{figure}

    %     In an attempt to retain the dependence structure during imputation, we investigated a copula based approach proposed by \citet{DiLascio2015}. \citet{DiLascio2015} test their method in the bivariate setting, however, applying this in the multivariate setting resulted in poor imputation. \citet{Hasler2018} propose an imputation method that utilises vine copulas. However, this method requires a monotonic non-response pattern, which our data does not have, nor can we restructure the data to create such a pattern. Relaxing this assumption to a random non-response pattern is an ongoing question and could be beneficial in this case.

    %     Given that we want to predict quantiles of the response given some set of covariates for C1 and C2, we felt the dependence structure needs to be unperturbed by the imputation method. We were unable to retain the dependence structure in the imputation process so we elected not to impute the data. To minimise the data loss, we decided to use available case analysis, so that only when a covariate of interest is missing will the observation be discarded. Under the model chosen in Section \ref{section: models_C1}, this will only result in c4\% of the data being discarded. \ED{c4\%? Also maybe we move this to the results section so we don't have to forward reference? Happy to discuss :)}

    As noted in \citet{Rohrbeck2023}, 11.7\% of the observations have at least one possible predictor variable $(V_{1}, V_{2}, V_{3}, V_{4}, V_{6}, V_{7})$ missing completely at random (MCAR). A detailed breakdown of the pattern of missing predictor observations is provided in the Supplementary Material. Since we can assume the data are MCAR, ignoring the observations that have a missing predictor variable will not bias our inference. However, a complete case analysis is undesirable due to the amount of data loss. To mitigate against this, we attempt to impute the observations where predictors are missing so they do not need to be discarded; see \citet{Little2019} for imputation techniques. For our purposes, the main aim is to ensure the imputation model does not alter the extremal dependence structure between the predictors and response. Neither of the methods we try, Multiple Imputation by Chained Equations \citep{vanBuuren2011}, and a copula-based approach proposed by \citet{DiLascio2015}, achieve this. Thus, to mitigate against the data loss, we use a case analysis rather than complete case analysis approach i.e., an observation will only be removed if the predictor is included in our model and its value is missing. This results in only 4.0\% of the data being discarded for our final model.

==> Sections/C1C2/model_development.tex <==
%%%% Threshold selection
In this section, we explain our model development procedure for $Y\mid\boldsymbol{X}$. We use a non-stationary GPD model \eqref{eqn:gpd_non_stationary} and detail the threshold and model selection in this section. This requires threshold selection and comparison of different covariate-dependent GPD parameterisations. Recall that we utilise the same model formulation for both C1 and C2 via~\eqref{eq:MC_dist}.  

When fitting a GPD, the first challenge is to select an appropriate threshold. 
% This selection involves a bias-variance trade-off: too low a threshold is likely to violate the asymptotic basis of the model, incorporating bias in the GPD fit, whereas higher threshold choices lead to additional uncertainty due to fewer exceedances being used to fit the model. A variety of methods exist which aim to balance this trade-off; \citet{Scarrott2012} provide a review and more recent developments include \citet{Northrop2017} and \citet{schneider2021threshold}. Owing to its favourable properties for IID data, 
We employ the threshold selection method of \citet{murphy2024automated} and extend this approach to select a threshold for non-stationary, covariate-dependent GPD models. The method selects a threshold based on minimising the expected quantile discrepancy (EQD) between the sample quantiles and fitted GPD model quantiles. When fitting a non-stationary model, the excesses will not be identically distributed across covariates. Thus, to utilise the EQD method in this case, we use the fitted non-stationary GPD parameter estimates to transform the excesses to common standard exponential margins and compare sample quantiles against theoretical quantiles from the standard exponential distribution. 

%\AF{The focus of challenges C1 and C2 is extreme quantile estimation. Thus, we elect to model $Y\mid\boldsymbol{X}$ using a non-stationary GPD model detailed in equation \eqref{eqn:gpd_non_stationary}. When fitting a GPD, the first challenge is to select an appropriate threshold. \citet{Scarrott2012} provide a review of the numerous methods one can use to choose the threshold and more recent developments include \citet{Northrop2017} and \citet{schneider2021threshold}. We employ the threshold selection method of \citet{murphy2024automated}, and extend their approach to a setting with non-stationary, covariate-dependent GPD models. Since the excesses will not be identically distributed across covariates, we compare thresholds minimising the expected quantile discrepancy (EQD) on standard exponential margins.}

Owing to the complex covariate structure observed in the data, as described in Section \ref{subsec:edac1andc2}, we employ the flexible EVGAM framework proposed in \citet{Youngman2019} for modelling GPD tail behaviour. Under this framework, GAM formulations are used to capture non-stationarity in the threshold, scale and shape functions introduced in Section \ref{subsec::background_EVA}. %In general, GAMs provide flexible functional forms that allow us to capture multiple covariate interactions. Moreover, both discrete and continuous covariates can be incorporated in the GAM framework. 

Without loss of generality, consider the scale function $\sigma(\boldsymbol{x})$. We assume that 
\begin{myequation}
    h(\sigma(\boldsymbol{x})) = \psi_\sigma(\boldsymbol{x}), \quad
\text{with} \quad    \psi_{\sigma}(\boldsymbol{x}) = \beta_0 + \sum\limits_{\kappa=1}^{K}\sum\limits_{p=1}^{P_{\kappa}} \beta_{\kappa p}b_{\kappa p} (\boldsymbol{x}),
    \label{eqn:general_gam_form}
\end{myequation}%\CB{What is $p$ in the sum?}
where $h(x) := \log(x)$ denotes the link function which ensures the correct support, with coefficients $\beta_0,\beta_{\kappa p} \in \RR$ and basis functions $b_{\kappa p}$ for $p \in \{1, \hdots, P_{\kappa}\}, \kappa \in \{1, \hdots, K\}$. \CBnew{Note that the basis functions can be in terms of individual covariates, i.e., $b_{\kappa p}:\RR \mapsto \RR$, or multiple covariates, i.e., $b_{\kappa p}:\RR^m \mapsto \RR$, $1 < m \leq 8$.} Analogous forms are taken for $v(\boldsymbol{x})$ and $\xi(\boldsymbol{x})$, adjusting the link function $h$ as appropriate, with $\psi_v$ and $\psi_{\xi}$ denoting the respective formulations.

For all GAM formulations, model fitting is carried out using the \verb|evgam| software package \citep{Youngman2022}, whereby restricted maximum likelihood estimation (REML) is used to approximate the GAM coefficients. \CBnew{Furthermore, we opt to only consider basis functions of singular covariates, since specifying basis functions of multiple variables requires a detailed understanding of covariate interactions and can significantly increase the computational complexity of the modelling procedure \citep{Wood2017}.}
%In general, REML schemes avoid over-fitting through penalisation of the likelihood function. Furthermore, formulation via likelihood functions avoids the use of Markov Chain Monte-Carlo methods, which can be computationally expensive; see \citet{Wood2017} for further details. 




% Letting $v(\boldsymbol{x})$, $\sigma(\boldsymbol{x}), \xi(\boldsymbol{x})$ are given as GAM formulations and uses fixed link functions which relate to a basis representation, denoted $\psi_*$. These link functions ensure that each parameter has the correct support and are given by:
% \begin{myequation}
%     \log \sigma(\boldsymbol{x}) = \psi_\sigma(\boldsymbol{x}) \quad \text{and} \quad \xi(\boldsymbol{x}) = \psi_\xi(\boldsymbol{x}), \quad
% \text{where} \quad    \psi_*(\boldsymbol{x}) = \beta_0 + \sum\limits_{\kappa=1}^{K}\sum\limits_{p=1}^{P_{\kappa}} \beta_{\kappa p}b_{\kappa p} (\boldsymbol{x})
%     \label{eqn:general_gam_form}
% \end{myequation}%\CB{What is $p$ in the sum?}
% with $\beta_{\kappa p}$ and $b_{\kappa p}$ denoting basis coefficients and functions, respectively. As a result, any likelihood resulting from \eqref{eqn: gpd_non_stationary}, now corresponds to estimating a set of basis coefficients $\beta_{kd}$. To control the smoothness of the GAM formulations and prevent overfitting, a penalised likelihood $L(\boldsymbol{\beta}_{\gamma})$ is used to estimate the basis coefficients \citep{Wood2017}. The corresponding log-likelihood $l(\boldsymbol{\beta_{\gamma}})$ is of the form: 
% \begin{myequation*}
%     l(\boldsymbol{\beta_{\gamma}}, \boldsymbol{\gamma}) = l(\boldsymbol{\beta_{\gamma}}) - \frac{1}{2} \boldsymbol{\beta}^T \boldsymbol{C_{\gamma} \beta}
% \end{myequation*}
% where $\boldsymbol{\gamma} = (\gamma_1, \ldots, \gamma_K)$ denotes the smoothing parameters, and $\boldsymbol{C_{\gamma}}$ is the penalty matrix with elements determined by $b_{\kappa p}$.

% Let $\log( u_{\tau}(\boldsymbol{\omega},\boldsymbol{x}_t)) = \psi_u(\boldsymbol{x}_t)$, $\log( \sigma\left(\boldsymbol{\omega} \mid \boldsymbol{x}_t\right)) = \psi_{\sigma}(\boldsymbol{x}_t)$ and $\xi\left(\boldsymbol{\omega} \mid \boldsymbol{x}_t\right) = \psi_{\xi}(\boldsymbol{x}_t)$ denote the GAM formulations of each function, where $\psi_{-}$ denotes the basis representation of equation \eqref{eqn:general_gam_form}. Exact forms of basis functions are specified in Section \ref{subsubsec:diagnostics_C3}. As in Section \ref{section:model_development}, model fitting is carried out using the \verb|evgam| software package \citep{Youngman2022}. For the first stage, $u_{\tau}(\boldsymbol{\omega},\boldsymbol{x}_t)$ is estimated using a likelihood-based inference procedure which exploits a link between the titled loss function, typically used in quantile regression, and the asymmetric Laplace distribution \citep{Yu2001}, allowing one to estimate the coefficients associated with $\psi_u$ in a relatively fast and objective manner. Estimation of $\psi_u$ is achieved via restricted maximum likelihood estimation (REML), with subsequent estimation of $\psi_{\sigma}$ and $\psi_{\xi}$ is also carried out in a similar manner. In general, REML schemes avoid over-fitting through penalisation of the likelihood function, as noted in Section \ref{section:model_development} \CB{Not removing this stuff yet, we just need to make sure it's covered when GAMs are first introduced}. Furthermore, formulation via likelihood functions avoids the use of MCMC, which can be computationally expensive; see \citet{Wood2017} and \citet{Youngman2019} for further details. 

% \subsubsection{Selection of GAM formulations and diagnostics} \label{subsubsec:diagnostics_C3}
% Prior to estimation of the threshold and parameter functions, we are first required to select a quantile level $\tau$ and formulations for each of the GAMs. To begin, we fix $\tau=0.9$ and restrict attention to the latter problem; this in turn involves selecting basis functions, basis dimensions and knot locations. As noted in \citet{Wood2017}, the most important choice here is the basis dimension; this corresponds with the flexibility of the resulting formulation. In practice, it is better to select a higher dimension than one would expect to be necessary, since the REML scheme will adjust estimates of coefficients to avoid over-fitting. Furthermore, as long as the basis dimension is sufficiently high, the locations of knots has little impact on the resulting model fits. \CB{Merge with Conor's}

% This is implemented via the \verb=evgam= package 

% that allows the model parameters to take the form of GAMs, enabling complex non-stationary relationships between the response and covariates to be captured. 
% Assuming that  $\sigma(\boldsymbol{x}), \xi(\boldsymbol{x})$ are given as GAM formulations and use fixed link functions which relate to a basis representation, denoted $\psi_*$. This link functions ensure that each parameter has the correct support and are given by:
% \begin{myequation}
%     \log \sigma(\boldsymbol{x}) = \psi_\sigma(\boldsymbol{x}) \quad \text{and} \quad \xi(\boldsymbol{x}) = \psi_\xi(\boldsymbol{x}), \quad
% \text{where} \quad    \psi_*(\boldsymbol{x}) = \beta_0 + \sum\limits_{\kappa=1}^{K}\sum\limits_{p=1}^{P_{\kappa}} \beta_{\kappa p}b_{\kappa p} (\boldsymbol{x})
%     \label{eqn:general_gam_form}
% \end{myequation}%\CB{What is $p$ in the sum?}
% with $\beta_{\kappa p}$ and $b_{\kappa p}$ denoting basis coefficients and functions, respectively. As a result, any likelihood resulting from \eqref{eqn: gpd_non_stationary}, now corresponds to estimating a set of basis coefficients $\beta_{kd}$. To control the smoothness of the GAM formulations and prevent overfitting, a penalised likelihood $L(\boldsymbol{\beta}_{\gamma})$ is used to estimate the basis coefficients \citep{Wood2017}. The corresponding log-likelihood $l(\boldsymbol{\beta_{\gamma}})$ is of the form: 
% \begin{myequation*}
%     l(\boldsymbol{\beta_{\gamma}}, \boldsymbol{\gamma}) = l(\boldsymbol{\beta_{\gamma}}) - \frac{1}{2} \boldsymbol{\beta}^T \boldsymbol{C_{\gamma} \beta}
% \end{myequation*}
% where $\boldsymbol{\gamma} = (\gamma_1, \ldots, \gamma_K)$ denotes the smoothing parameters, and $\boldsymbol{C_{\gamma}}$ is the penalty matrix with elements determined by $b_{\kappa p}$.

%%%%%%%%%%%%%%%%%%%%% CV
For model performance assessment and selection, we apply $k$-fold CV \citep[Ch 7.]{Hastie2008}. 
%This allows us to establish how well the model performs on out-of-sample data while avoiding over-fitting \citep[Ch 7.]{Hastie2008}. 
We divide the data into $k$ groups (folds), where each fold is removed in turn and the model is fitted to the remaining data. Choosing a higher number $k$ provides less biased CV metrics with a higher variance. A lower $k$ is computationally cheaper, however, it may overestimate the test error rate. We explore model ranking by taking both $k = 10$ and $50$, and find that both give an equivalent ranking; we present results for the latter. For each omitted fold, we compute several goodness-of-fit measures: Akaike Information Criterion (AIC), Bayesian Information Criterion (BIC), and the continuous ranked probability score \citep[CRPS,][]{Gneiting2014}. AIC and BIC aid in guiding the model search, favouring parsimony by penalising model complexity, while %Unlike root mean square error (RMSE) \CB{Do we need to mention RMSE??},
%evaluates the closeness between the empirically estimated and predicted quantiles, while 
CRPS describes the discrepancy between the predicted distribution function and observed values without the specification of empirical quantiles.
% \citep{Zamo2018}.
%which is non-trivial in temporally non-stationary settings, which our data exhibits.\CB{Would cut from comma.}. 
Finally, we report the average criterion over all 50 folds for each model; lower values of AIC, BIC and CRPS indicate a better model fit.

\subsubsection{Model selection} \label{subsubsec:model_sel}
Our analysis in Section \ref{subsec:edac1andc2} indicates that $V_{3}$, $V_{5}$ (season), and $V_{6}$ (wind speed) exhibit non-trivial dependence relationships with the response variable; we therefore assume these variables can be used as predictor variables for modelling $Y$, and set $\Tilde{\boldsymbol{X}} := (\boldsymbol{V}_{j})_{j\in \{3,5,6\}}$, with $\Tilde{X}_{r,t}$ denoting the $r^{\text{th}}$ component of $\Tilde{\boldsymbol{X}}$, $r \in \{1,2,3\}$. Although $V_{7}$ (wind direction) also exhibits predictor power, we have not considered it here since it is highly correlated with wind speed so would involve adding complex interaction terms to the model formulation, and $V_6$ has a stronger relationship with $Y$ compared to $V_7$ (see Figure~\ref{fig:dep_heat}). 

There is a clear variation in the distribution of $Y$ between seasons. Due to this distinct difference, we explore the inclusion of a stepped-threshold according to season. In particular, we set $v(\Tilde{\boldsymbol{x}}_t):= \mathbbm{1}(\Tilde{x}_{2,t} = 1)v_1 + \mathbbm{1}(\Tilde{x}_{2,t} = 2)v_2$, $v_1,v_2 \in \RR$, with corresponding rate parameter $\lambda(\Tilde{\boldsymbol{x}}_t):= \mathbbm{1}(\Tilde{x}_{2,t} = 1)\lambda_1 + \mathbbm{1}(\Tilde{x}_{2,t} = 2)\lambda_2$, where $\lambda_1, \lambda_2 \in [0,1]$ denote the non-exceedance probabilities for seasons $1$ and $2$, respectively. This seasonal threshold significantly improves model fits; see the Supplementary Material for further details. GAM forms for the threshold were also explored, but did not offer significant improvement. Furthermore, the smooth GAM formulation of the GPD scale parameter adequately captures any residual variation in the response arising due to covariate dependence. 

%%%% Choosing covariates and their forms
Using the \verb|evgam| package, we fit the non-stationary GPD to the tail of $Y$, with $\sigma(\boldsymbol{x})$ as in equation \eqref{eqn:general_gam_form}. We keep the shape function $\xi(\boldsymbol{x}):=\xi \in \RR$ constant across covariates; this is common in non-stationary analyses, since this parameter is difficult to estimate \citep{Chavez-Demoulin2005}.
% , which would increase the complexity of the modelling procedure substantially. 
%%%%%%% Forms for covariate %%%
Even after accounting for seasonal variability in the threshold, including the seasonal variable in the scale function formulation via an indicator function improves model fits. 

%From Section \ref{subsec:edac1andc2}, we know there is a step change in the mean for $V_{6}$; we consider both an indicator function and a spline to capture the relationship between $Y$ and this predictor. 
When using splines, we are required to select a basis dimension $B \in \NN$; this determines the number of coefficients to be estimated. Basis dimension is the most important choice within spline modelling procedures and directly corresponds with the flexibility of the framework \citep{Wood2017}. %In practice, it is better to select a higher dimension than we would expect to be necessary since the REML scheme will adjust estimates of coefficients to avoid over-fitting. Furthermore, as long as the basis dimension is sufficiently high, the locations of knots have little impact on the resulting model fits. Note that we use thin-plate regression splines as they can smooth with respect to any number of covariates, and it is the default in the \verb|evgam| package \citep{Youngman2022}. Other types of splines could be used, but we do not consider them here. 
To determine $B$ for $V_{6}$, we build a model for $Y \mid \Tilde{X}_{3}$, allowing us to consider the effect of this predictor on the response directly. We vary the basis dimension, and compare the resulting models using CV. Through this, we set $B=3$ since this appears to offer sufficient flexibility to capture the observed dependence. For $V_3$, we employ a similar procedure and set $B=4$. 





==> Sections/C1C2/model_selection.tex <==
% To determine the best-fitting model, we use a forward selection process based on minimising the CV score using CRPS. Specifically, by comparing model fits with only a single predictor variable (models 2-4 in Table \ref{tab:C1_Models}), we find model 4 minimises the CV score and so we add $V_{3}$ to the model. Continuing in this fashion results in our final model being model 7. Wind speed ($V_{6}$) was also modelled using an indicator function to try and capture its changepoint although this did not improve the model fit and has been omitted in Table \ref{tab:C1_Models}. We have omitted models that included additional predictor variables and interaction terms as they do not reduce the CV score further.

To determine the best-fitting model, we use a forward selection process based on minimising the CV score using CRPS. Selected models used in the forward selection process are detailed in Table \ref{tab:C1_Models}) until the CRPS is minimised giving us our final model, model 7. Let $y_{t}$ and $\Tilde{\boldsymbol{x}}_t$ denote the observations of the response variable and predictive covariates, respectively. Then our model has the following form, 
\begin{myequation}
    F_{Y_t|\Tilde{\boldsymbol{X}}_t}(y_{t} | \Tilde{\boldsymbol{X}}_t = \Tilde{\boldsymbol{x}}_t, y_{t} > v(\Tilde{\boldsymbol{x}}_t)) = 1-\lambda(\Tilde{\boldsymbol{x}}_t)\left[1+\xi\left(\frac{y_{t}-v(\Tilde{\boldsymbol{x}}_t)}{\sigma(\Tilde{\boldsymbol{x}_t})}\right)\right]_+^{-1/\xi}, \label{eq:C1_model}
\end{myequation}
for all $t \in \{1,\hdots,n\}$. The formulation of $\sigma(\cdot)$ is defined in Table~\ref{tab:C1_Models} as model 7, 
% \begin{myequation}
%     \sigma(\Tilde{\boldsymbol{x}}_t) = \beta_0 + \beta_{1} \mathbbm{1}(\Tilde{x}_{2,t}=1) + s_{2}(\Tilde{x}_{1,t}) + s_{3}(\Tilde{x}_{3,t}),
% \end{myequation}
where $\beta_0,\beta_{1}\in\mathbb{R}$ denote coefficients, and $s_{1}, s_{2}$ are thin-plate regression splines for $V_3$ and $V_6$, respectively, with corresponding basis coefficients $\boldsymbol{\beta}_{2}\in\mathbb{R}^{3}$ and $\boldsymbol{\beta}_{3}\in\mathbb{R}^{4}$.

%%%%%%%%%%%%%%%%%% Table
\begin{table}[h!]
\caption{Table of selected models considered for challenge C1. $\mathbbm{1}(\cdot)$ denotes an indicator function, $s_{i}(\cdot)$ for $i \in \{1,2\}$ denote thin-plate regression splines, $\beta_0,\beta_1$ are coefficients to be estimated, and $\tilde{{x}}_{r,t}$ is defined as in the text. All values have been given to one decimal place.}
\centering
\vspace{0.5em}
\begin{tabular}{l|l|l|l|l}
\toprule
Model & $\sigma(\tilde{\boldsymbol{x}}_{t})$ & CRPS & AIC & BIC \\
\hline
1 & $\beta_{0}$ & 11.5 & 92,059.9 & 92,074.5 \\
\hline
2 & $\beta_{0} + \beta_{1} \mathbbm{1}(\tilde{x}_{2,t} = 1)$ & 11.0 & 92,026.5 & 92,048.4 \\
\hline
3 & $\beta_{0} + s_{1}(\tilde{x}_{1,t})$ & 10.6 & 91,651.4 & 91,695.3 \\
\hline
4 & $\beta_{0} + s_{2}(\tilde{x}_{3,t})$ & 11.0 & 91,775.6 & 91,797.7 \\
\hline
5 & $\beta_{0} + \beta_{1} \mathbbm{1}(\tilde{x}_{2,t} = 1) + s_{1}(\tilde{x}_{1,t})$ & 10.6 & 91,634.1 & 91,686.4 \\
\hline
6 & $\beta_{0} + s_{1}(\tilde{x}_{1,t}) + s_{2}(\tilde{x}_{3,t})$ & 10.5 & 91,307.2 & 91,357.3 \\
\hline
7 & $\beta_{0} + \beta_{1} \mathbbm{1}(\tilde{x}_{2,t} = 1) + s_{1}(\tilde{x}_{1,t}) + s_{2}(\tilde{x}_{3,t})$ & \textbf{10.4} & \textbf{91,279.9} & \textbf{91,339.2} \\
\bottomrule 
\end{tabular}

\label{tab:C1_Models}
\end{table}

==> Sections/C1C2/penalised_likelihood.tex <==
For challenge C2, we 
%are required to 
incorporate the loss function of equation \eqref{eq:loss_fn} into the modelling framework. Letting $\mathcal{I}_v := \{ t \in \{1,\hdots,n\} \mid y_t > v(\Tilde{\boldsymbol{x}}_t) \}$ and $n_v := | \mathcal{I}_v |$, we consider the following objective function
\begin{myequation*}
    S(\boldsymbol{\theta}) := - l_R(\boldsymbol{\theta}) + \sum\limits_{i\in\mathcal{I}_v} \mathcal{L}(q_i^*, \hat{q}_i)/n_v,
\end{myequation*}
where $l_R(\boldsymbol{\theta})$ denotes the penalised log-likelihood function of the REML approach \citep{Wood2017}, $\boldsymbol{\theta}:= (\beta_0,\beta_1,\bm{\beta}_{2},\bm{\beta}_{3},\xi)$ denotes the parameter vector associated with the GPD formulation, and $\sum\limits_{i\in\mathcal{I}_v} \mathcal{L}(q_i^*, \hat{q}_i)/n_v$ denotes the average loss between the sample quantiles of the transformed excesses and the theoretical standard exponential quantiles. Specifically, we transform the excesses, $(y_{t} - v(\Tilde{\boldsymbol{x}}_t))_{t \in \mathcal{I}_v}$, to standard exponential margins using the fitted non-stationary GPD parameter estimates and compare the ordered excesses, $\bm{q}^*$, to the theoretical quantiles, $\hat{\bm{q}}$, from a standard exponential distribution evaluated at probabilities $\{p_i = i/(n_v + 1), i=1, \ldots, n_v\}$.
%if we denote the mapping between $\mathcal{I}_v$ and the order statistics of $(y_{t} - v(\Tilde{\boldsymbol{x}}_t))_{t \in \mathcal{I}_v}$ by $\pi,$ then $q_i^*$ is the $\pi(i)$\textsuperscript{th} order statistic of $(y_{t} - v(\Tilde{\boldsymbol{x}}_t))_{t \in \mathcal{I}_v}$ and $\hat{q}_i =  \sigma(\bm{x}_{\pi(i)})[\{ 1 - \pi(i)/(n_v + 1)  \}^{-\xi}-1]/\xi$.
Minimising $S(\boldsymbol{\theta})$ ensures the parameter estimates also account for the loss function. We use this formulation to adjust the GPD parameters for challenge C2 once a threshold is selected.

% Letting $\mathcal{I}_v := \{ t \in \{1,\hdots,n\} \mid y_t > v_t \}$, we approximate $\mathbb{E}_{\bm{q}^*}\left[\mathcal{L}(\bm{q}^*, \hat{\bm{q}})\right] = \sum\limits_{i=1}^{n_v} \mathcal{L}(q_i^*, \hat{q}_i)/n_v$, where $n_v := | \mathcal{I}_v |$, and $q_i^*$ and $\hat{q}_i$ denote the theoretical and empirical GPD quantiles, respectively, i.e.,  $q_i^*$ denotes the $i$-th order statistic of  $(y_{t} - v_t)_{t \in \mathcal{I}_v}$ and $\hat{q}_i =  \sigma(x_i)[(1- 1/(i + 1) )^{-\hat{\xi}}-1]/\hat{\xi}$.  }


% The expectation is calculated over the sample quantiles $q_i^* = (p_i, y^{(i)}_v)$ with $\{p_i = i / (n_v+1): i = 1,\dots,n_v\}$ and $y^{(i)}_v$ denoting the $i^{\text{th}}$ order statistic of $\bm{y}_v$ (increasing with $i$). For each $q^*_i$, we use the fitted GPD model to estimate the corresponding $\hat{q}_i =  \hat{\sigma}(x_i)[(1-p_i)^{-\hat{\xi}}-1]/\hat{\xi}$. We use this formulation to adjust the GPD parameters for challenge C2 once a threshold is selected.  

% % Letting $\mathcal{I}_v := \{ t \in \{1,\hdots,n\} \mid y_t > v_t \}$ denote the indices of threshold exceeding values, 


% Let $\boldsymbol{y}_v = (y_1, \ldots, y_{n_v})$ denote the set of $n_v$ exceedances with threshold $v$. To incorporate this loss function \eqref{eq:loss_fn} into our GPD model~\ref{eq:C1_model}, we used a penalised likelihood of the following form: \CM{If I have defined the threshold $v$ as stepped, do I need an indicator in this likelihood or is just $v$ okay? Or $v_{\text{step}}$ or something?}
% \begin{myequation}
% \label{eqn: gpdll}
%     l(\sigma(\bm{x}),\xi) = -\sum\limits_{i=1}^{n_v}\left\{\log(\sigma(x_i)) + (1 + 1/\xi) \log\left(1 + \frac{\xi (y_i - v)}{\sigma(x_i)}\right)\right\} + \phi \mathbb{E}_{\bm{q}^*}\left[\mathcal{L}(\bm{q}^*, \hat{\bm{q}})\right],
% \end{myequation} 
% \AF{think we need to update the index. Is $i$ the $i^{\text{th}}$ observation or the $i^{\text{th}}$ threshold?}
% \AF{Should $\sigma(x_{i})$ not be $\boldsymbol{\sigma}(\mathbf{x}_{i})$?}
% provided $(1 + \xi (y_i - v)/\sigma(x_i)) > 0$ for $i = 1,\ldots,n_v$. Otherwise, $l(\sigma(\bm{x}),\xi) = -\infty$.

% In this model formulation, $\phi$ denotes the penalty term which penalises according to the expected loss $\mathbb{E}_{\bm{q}^*}\left[\mathcal{L}(\bm{q}^*, \hat{\bm{q}})\right]= \sum\limits_{i=1}^{n_v} \mathcal{L}(q_i^*, \hat{q}_i)/n_v$. The expectation is calculated over the sample quantiles $q_i^* = (p_i, y^{(i)}_v)$ with $\{p_i = i / (n_v+1): i = 1,\dots,n_v\}$ and $y^{(i)}_v$ denoting the $i^{\text{th}}$ order statistic of $\bm{y}_v$ (increasing with $i$). For each $q^*_i$, we use the fitted GPD model to estimate the corresponding $\hat{q}_i =  \hat{\sigma}(x_i)[(1-p_i)^{-\hat{\xi}}-1]/\hat{\xi}$.



==> Sections/C1C2/results.tex <==
For C1, we use our final model of Section~\ref{section:model_development} to estimate the 0.9999-quantile of $Y\mid\tilde{\boldsymbol{X}} = \tilde{\boldsymbol{x}_{i}}$, $i \in \{1,\hdots,100\}$, for the set of 100 covariate combinations. The left panel of Figure \ref{fig:C1_Results} shows the quantile-quantile (QQ) plot for our model. There is general alignment between the model and empirical quantiles; however, there is some under-estimation in the upper tail, and our 95\% tolerance bounds do not contain some of the most extreme response values. The right panel of Figure \ref{fig:C1_Results} shows our predicted quantiles, and their association confidence intervals, compared to their true quantiles. This figure is different from the one presented by \citet{Rohrbeck2023} due to an error in our code being fixed after submission. In this scenario, our estimated confidence intervals lead to a $14\%$ coverage of the true quantiles, which does not alter our ranking for this challenge. Our performance and model improvements are discussed in Section \ref{sec:discussion}.

\begin{figure}
     \centering
     \begin{subfigure}[h]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Aiden/231120_QQ_plot_Model_13.pdf}
         \label{fig:231120_QQ_plot_Model_13}
     \end{subfigure}
     \begin{subfigure}[h]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Aiden/231123_Model_13_vs_Truth.pdf}
         \label{fig:231123_C1_Results}
     \end{subfigure}
     \caption{QQ plot for our final model, model 7 in Table \ref{tab:C1_Models}, on exponential margins. The $y=x$ line is given in red and the grey region represents the 95\% tolerance bounds (left). Predicted $0.9999-$quantiles against true quantiles for the 100 covariate combinations. The points are the median predicted quantile over 200 bootstrapped samples and the vertical error bars are the corresponding 50\% confidence intervals. The $y = x$ line is also shown (right).} 
    \label{fig:C1_Results}
\end{figure}

For challenge C2, we estimate the quantile of interest as %$\hat q= 212.6 \; (208.4, 246.1)$ 
$\hat{q} = 213.1 \; (209.3, 242.1)$. Due to a coding error, this value differs from the original estimate submitted for the data challenge. The updated estimate over-estimates compared to the truth. A 95\% confidence interval for the estimate is given in parentheses based on the bootstrapping procedure outlined in Section~\ref{section:uncertainty}. %Our estimate overestimates the true quantile and ranks 4$^{\text{th}}$ for the C2 subchallenge~\citep{Rohrbeck2023}.
